The Mass Distribution and Lifetime of Prestellar Cores in Perseus, Serpens, and Ophiuchus

We present an unbiased census of starless cores in Perseus, Serpens, and Ophiuchus, assembled by comparing large-scale Bolocam 1.1 mm continuum emission maps with Spitzer c2d surveys. We use the c2d catalogs to separate 108 starless from 92 protostellar cores in the 1.1 mm core samples from Enoch et al. (2006), Young et al. (2006), and Enoch et al. (2007). A comparison of these populations reveals the initial conditions of the starless cores. Starless cores in Perseus have similar masses but larger sizes and lower densities on average than protostellar cores, with sizes that suggest density profiles substantially flatter than r^-2. By contrast, starless cores in Serpens are compact and have lower masses than protostellar cores; future star formation will likely result in lower mass objects than the currently forming protostars. Comparison to dynamical masses estimated from the NH_3 survey of Perseus cores by Rosolowsky et al. (2007) suggests that most of the starless cores are likely to be gravitationally bound, and thus prestellar. The combined prestellar core mass distribution includes 108 cores and has a slope of -2.3+/-0.4 for M>0.8 Msun. This slope is consistent with recent measurements of the stellar initial mass function, providing further evidence that stellar masses are directly linked to the core formation process. We place a lower limit on the core-to-star efficiency of 25%. There are approximately equal numbers of prestellar and protostellar cores in each cloud, thus the dense prestellar core lifetime must be similar to the lifetime of embedded protostars, or 4.5x10^5 years, with a total uncertainty of a factor of two. Such a short lifetime suggests a dynamic, rather than quasi-static, core evolution scenario, at least at the relatively high mean densities (n>2x10^4 cm^-3) to which we are sensitive.

==> tab1.2.tex <==
\ProvidesFile{tab1.2.tex}

\begin{deluxetable*}{lccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Starless cores in Perseus, Serpens, and Ophiuchus\label{sltab}}
\tablehead{
\colhead{Bolocam ID } & \colhead{RA} & \colhead{Dec} & \colhead{Peak flux} & \colhead{Total mass} & \colhead{$\theta_{dec}$} & \colhead{Axis ratio} & \colhead{$n_{1e4}$} \\
\colhead{} & \colhead{(hr)} & \colhead{(deg)} & \colhead{(mJy/beam)} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{(arcsec)} & \colhead{} & \colhead{(cm$^{-3}$)}
}
\startdata
\hline
\multicolumn{8}{c}{Perseus}  \\
\hline
Per-Bolo 1  &  03 25 07.8  &  +30 24 22  &  109  &  0.28  & 30.4   & 1.5  & 0.9$\times 10^5$  \\ 
Per-Bolo 2  &  03 25 09.5  &  +30 23 51  &  121  &  0.36  & 15.7   & 1.6  & 1.1$\times 10^5$  \\ 
Per-Bolo 3  &  03 25 10.2  &  +30 44 43  &  125  &  0.92  & 85.5   & 2.1  & 1.0$\times 10^5$  \\ 
Per-Bolo 4  &  03 25 17.0  &  +30 18 53  &  149  &  2.99  & 104.9  & 1.2  & 1.5$\times 10^5$  \\ 
Per-Bolo 6  &  03 25 26.5  &  +30 21 50  &  143  &  2.85  & 105.6  & 1.4  & 1.3$\times 10^5$  \\ 
Per-Bolo 7  &  03 25 35.4  &  +30 13 06  &  126  &  2.32  & 98.1   & 1.4  & 1.1$\times 10^5$  \\ 
Per-Bolo 9  &  03 25 37.2  &  +30 09 55  &  113  &  1.70  & 98.2   & 1.9  & 1.0$\times 10^5$  \\ 
Per-Bolo 11  &  03 25 46.0  &  +30 44 10  &  241  &  2.18  & 72.5  & 1.0  & 2.2$\times 10^5$  \\ 
Per-Bolo 12  &  03 25 47.5  &  +30 12 26  &  118  &  2.34  & 95.6  & 1.8  & 1.1$\times 10^5$  \\ 
Per-Bolo 13  &  03 25 48.8  &  +30 42 24  &  407  &  1.14  & 38.2  & 1.3  & 3.9$\times 10^5$  \\ 
Per-Bolo 14  &  03 25 50.6  &  +30 42 01  &  342  &  1.00  & 38.7  & 1.4  & 3.5$\times 10^5$  \\ 
Per-Bolo 15  &  03 25 55.1  &  +30 41 26  &  188  &  0.60  & 46.6  & 1.1  & 1.7$\times 10^5$  \\ 
Per-Bolo 16  &  03 25 56.2  &  +30 40 41  &  154  &  0.50  & 44.8  & 1.1  & 1.5$\times 10^5$  \\ 
Per-Bolo 17  &  03 25 58.4  &  +30 37 13  &  122  &  0.88  & 65.9  & 1.2  & 0.9$\times 10^5$  \\ 
Per-Bolo 19  &  03 27 02.0  &  +30 15 08  &  115  &  1.42  & 83.3  & 1.1  & 1.1$\times 10^5$  \\ 
Per-Bolo 20  &  03 27 28.8  &  +30 15 02  &  114  &  1.67  & 80.8  & 1.4  & 1.1$\times 10^5$  \\ 
Per-Bolo 26  &  03 28 32.4  &  +31 04 43  &  117  &  1.28  & 65.5  & 1.5  & 1.2$\times 10^5$  \\ 
Per-Bolo 32  &  03 28 41.7  &  +30 31 13  &  144  &  1.84  & 94.8  & 1.1  & 1.1$\times 10^5$  \\ 
Per-Bolo 33  &  03 28 42.6  &  +31 06 12  &  173  &  0.65  & 46.2  & 1.1  & 1.9$\times 10^5$  \\ 
Per-Bolo 34  &  03 28 45.9  &  +31 15 20  &  147  &  0.56  & 33.0  & 1.4  & 1.3$\times 10^5$  \\ 
Per-Bolo 44  &  03 29 04.5  &  +31 18 42  &  274  &  1.73  & 47.0  & 1.7  & 2.7$\times 10^5$  \\ 
Per-Bolo 45  &  03 29 07.7  &  +31 17 17  &  455  &  3.25  & 52.9  & 1.3  & 4.8$\times 10^5$  \\ 
Per-Bolo 50  &  03 29 14.5  &  +31 20 30  &  313  &  3.15  & 68.0  & 1.2  & 3.2$\times 10^5$  \\ 
Per-Bolo 51  &  03 29 17.0  &  +31 12 26  &  423  &  1.49  & 34.7  & 1.4  & 3.6$\times 10^5$  \\ 
Per-Bolo 55  &  03 29 19.4  &  +31 11 37  &  184  &  0.89  & 40.0  & 1.3  & 2.1$\times 10^5$  \\ 
Per-Bolo 56  &  03 29 22.4  &  +31 36 24  &  102  &  1.41  & 83.7  & 1.3  & 1.0$\times 10^5$  \\ 
Per-Bolo 58  &  03 29 25.7  &  +31 28 16  &  273  &  0.78  & 25.9  & 1.2  & 1.8$\times 10^5$  \\ 
Per-Bolo 61  &  03 30 24.0  &  +30 27 39  &  106  &  0.89  & 68.9  & 1.8  & 0.8$\times 10^5$  \\ 
Per-Bolo 63  &  03 30 45.5  &  +30 52 34  &  141  &  1.61  & 79.0  & 1.1  & 1.5$\times 10^5$  \\ 
Per-Bolo 64  &  03 30 50.4  &  +30 49 17  &  86   &  0.49  & 36.5  & 2.2  & 0.7$\times 10^5$  \\ 
Per-Bolo 67  &  03 32 26.9  &  +30 59 11  &  165  &  2.07  & 64.0  & 2.7  & 1.6$\times 10^5$  \\ 
Per-Bolo 69  &  03 32 39.3  &  +30 57 29  &  155  &  3.09  & 113.5 & 1.2  & 1.2$\times 10^5$  \\ 
Per-Bolo 70  &  03 32 44.0  &  +31 00 00  &  238  &  4.74  & 97.2  & 1.2  & 2.4$\times 10^5$  \\ 
Per-Bolo 71  &  03 32 51.2  &  +31 01 48  &  184  &  2.77  & 83.4  & 1.3  & 2.0$\times 10^5$  \\ 
Per-Bolo 72  &  03 32 57.0  &  +31 03 21  &  235  &  2.23  & 61.8  & 1.4  & 2.3$\times 10^5$  \\ 
Per-Bolo 73  &  03 33 00.0  &  +31 20 44  &  178  &  2.68  & 93.9  & 1.3  & 1.6$\times 10^5$  \\ 
Per-Bolo 74  &  03 33 01.9  &  +31 04 32  &  255  &  0.91  & 44.5  & 1.2  & 2.6$\times 10^5$  \\ 
Per-Bolo 75  &  03 33 04.4  &  +31 04 59  &  259  &  0.91  & 45.0  & 1.2  & 2.6$\times 10^5$  \\ 
Per-Bolo 77  &  03 33 11.4  &  +31 17 24  &  110  &  0.92  & 76.6  & 1.3  & 0.9$\times 10^5$  \\ 
Per-Bolo 82  &  03 33 25.1  &  +31 05 35  &  147  &  0.88  & 47.7  & 1.1  & 1.4$\times 10^5$  \\ 
Per-Bolo 83  &  03 33 25.4  &  +31 20 07  &  165  &  1.14  & 57.9  & 1.2  & 1.5$\times 10^5$  \\ 
Per-Bolo 85  &  03 33 32.1  &  +31 20 04  &  155  &  0.96  & 54.9  & 1.4  & 1.3$\times 10^5$  \\ 
Per-Bolo 86  &  03 33 51.1  &  +31 12 37  &  131  &  1.53  & 96.7  & 1.7  & 0.9$\times 10^5$  \\ 
Per-Bolo 87  &  03 35 21.6  &  +31 06 55  &  99   &  1.09  & 75.6  & 1.5  & 0.9$\times 10^5$  \\ 
Per-Bolo 88  &  03 40 14.5  &  +32 01 30  &  162  &  3.44  & 114.4 & 1.6  & 1.5$\times 10^5$  \\ 
Per-Bolo 89  &  03 40 49.3  &  +31 48 35  &  151  &  2.40  & 95.0  & 1.6  & 1.4$\times 10^5$  \\ 
Per-Bolo 91  &  03 41 19.7  &  +31 47 28  &  106  &  0.88  & 69.3  & 1.8  & 0.9$\times 10^5$  \\ 
Per-Bolo 92  &  03 41 40.0  &  +31 58 05  &  94   &  0.57  & 50.3  & 1.2  & 0.9$\times 10^5$  \\ 
Per-Bolo 93  &  03 41 45.1  &  +31 48 10  &  118  &  2.16  & 95.6  & 1.2  & 1.2$\times 10^5$  \\ 
Per-Bolo 94  &  03 41 45.8  &  +31 57 22  &  132  &  0.77  & 52.4  & 1.2  & 1.1$\times 10^5$  \\ 
Per-Bolo 95  &  03 42 20.6  &  +31 44 49  &  108  &  1.85  & 98.5  & 1.2  & 0.9$\times 10^5$  \\ 
Per-Bolo 96  &  03 42 47.1  &  +31 58 41  &  148  &  1.10  & 55.3  & 1.2  & 1.5$\times 10^5$  \\ 
Per-Bolo 97  &  03 42 52.3  &  +31 58 12  &  149  &  0.85  & 53.8  & 1.1  & 1.6$\times 10^5$  \\ 
Per-Bolo 98  &  03 42 57.3  &  +31 57 49  &  134  &  0.77  & 52.1  & 1.1  & 1.4$\times 10^5$  \\ 
Per-Bolo 99  &  03 43 38.3  &  +32 03 09  &  164  &  1.04  & 46.5  & 1.2  & 1.7$\times 10^5$  \\ 
Per-Bolo 100  &  03 43 44.0  &  +32 03 10  &  250  &  1.95  & 53.7  & 1.1  & 2.8$\times 10^5$  \\ 
Per-Bolo 101  &  03 43 45.6  &  +32 01 45  &  139  &  0.84  & 45.0  & 1.4  & 1.4$\times 10^5$  \\ 
Per-Bolo 105  &  03 43 57.8  &  +32 04 06  &  283  &  1.47  & 46.6  & 1.3  & 2.8$\times 10^5$  \\ 
Per-Bolo 107  &  03 44 02.1  &  +32 02 34  &  388  &  1.17  & 46.0  & 1.1  & 4.1$\times 10^5$  \\ 
Per-Bolo 111  &  03 44 14.5  &  +31 58 00  &  170  &  2.00  & 77.7  & 1.4  & 1.5$\times 10^5$  \\ 
Per-Bolo 112  &  03 44 14.8  &  +32 09 13  &  127  &  1.09  & 53.3  & 1.1  & 1.2$\times 10^5$  \\ 
Per-Bolo 114  &  03 44 22.7  &  +32 10 01  &  140  &  1.32  & 63.5  & 1.5  & 1.3$\times 10^5$  \\ 
Per-Bolo 115  &  03 44 36.4  &  +31 58 39  &  167  &  1.30  & 53.0  & 2.1  & 1.5$\times 10^5$  \\ 
Per-Bolo 117  &  03 44 48.8  &  +32 00 30  &  150  &  0.97  & 42.9  & 1.6  & 1.5$\times 10^5$  \\ 
Per-Bolo 118  &  03 44 56.0  &  +32 00 31  &  109  &  0.81  & 52.7  & 1.9  & 1.0$\times 10^5$  \\ 
Per-Bolo 119  &  03 45 15.9  &  +32 04 48  &  181  &  3.11  & 101.0 & 1.3  & 1.6$\times 10^5$  \\ 
Per-Bolo 121  &  03 47 33.5  &  +32 50 55  &  136  &  1.57  & 83.2  & 1.1  & 1.3$\times 10^5$  \\ 
\vspace{0.1cm} \\
\hline
\multicolumn{8}{c}{Serpens}  \\
\hline
Ser-Bolo 1  &  18 28 23.1  &  +00 26 35  &  95   &  0.65  & 46.3  & 1.2  & 0.9$\times 10^5$  \\ 
Ser-Bolo 4  &  18 28 47.2  &  +00 50 45  &  145  &  0.73  & 35.3  & 1.3  & 1.5$\times 10^5$  \\ 
Ser-Bolo 5  &  18 28 48.3  &  +00 14 52  &  73   &  0.42  & 45.3  & 1.3  & 0.6$\times 10^5$  \\ 
Ser-Bolo 6  &  18 28 50.8  &  +00 50 29  &  115  &  0.55  & 41.5  & 1.3  & 1.2$\times 10^5$  \\ 
Ser-Bolo 10  &  18 28 56.6  &  +00 19 10  &  107  &  0.38  & 41.2  & 1.1  & 1.0$\times 10^5$  \\ 
Ser-Bolo 11  &  18 28 57.3  &  +00 48 07  &  162  &  0.52  & 30.2  & 1.6  & 1.6$\times 10^5$  \\ 
Ser-Bolo 12  &  18 28 58.4  &  +00 47 36  &  172  &  0.64  & 32.2  & 1.5  & 1.7$\times 10^5$  \\ 
Ser-Bolo 16  &  18 29 13.5  &  +00 32 13  &  175  &  0.71  & 37.5  & 1.5  & 1.5$\times 10^5$  \\ 
Ser-Bolo 18  &  18 29 19.3  &  +00 33 29  &  104  &  0.65  & 47.2  & 1.5  & 1.0$\times 10^5$  \\ 
Ser-Bolo 19  &  18 29 31.5  &  +00 26 49  &  279  &  3.34  & 74.2  & 1.2  & 2.8$\times 10^5$  \\ 
Ser-Bolo 21  &  18 29 43.4  &  +00 36 25  &  129  &  0.98  & 48.0  & 1.2  & 1.2$\times 10^5$  \\ 
Ser-Bolo 30  &  18 30 02.5  &  +01 15 25  &  319  &  1.13  & 39.6  & 1.1  & 2.9$\times 10^5$  \\ 
Ser-Bolo 31  &  18 30 02.8  &  +01 08 38  &  214  &  1.70  & 45.5  & 1.6  & 2.1$\times 10^5$  \\ 
Ser-Bolo 34  &  18 30 08.2  &  +01 13 12  &  153  &  0.56  & 34.3  & 1.5  & 1.2$\times 10^5$  \\ 
Ser-Bolo 35  &  18 30 14.7  &  +01 13 53  &  85   &  0.16  & 20.2  & 2.5  & 0.4$\times 10^5$  \\ 
\hline
\multicolumn{8}{c}{Ophiuchus}  \\
\hline
Oph-Bolo 1  &  16 25 59.1  &  -24 18 16  &  261  &  1.29  & 102.7 & 1.5  & 1.4$\times 10^5$  \\ 
Oph-Bolo 2  &  16 26 08.1  &  -24 20 01  &  388  &  0.28  & 46.2  & 1.1  & 2.7$\times 10^5$  \\ 
Oph-Bolo 3  &  16 26 09.6  &  -24 19 16  &  307  &  0.35  & 44.8  & 1.1  & 2.0$\times 10^5$  \\ 
Oph-Bolo 6  &  16 26 22.9  &  -24 20 01  &  274  &  0.35  & 53.7  & 1.1  & 1.2$\times 10^5$  \\ 
Oph-Bolo 10  &  16 26 29.7  &  -24 24 29  &  2664 &  2.07  & 36.8  & 1.3  & 13.7$\times 10^5$   \\ 
Oph-Bolo 13  &  16 27 04.3  &  -24 38 47  &  233  &  0.82  & 78.8  & 1.3  & 1.3$\times 10^5$  \\ 
Oph-Bolo 15  &  16 27 12.2  &  -24 29 19  &  437  &  0.56  & 45.8  & 1.3  & 2.4$\times 10^5$  \\ 
Oph-Bolo 16  &  16 27 15.1  &  -24 30 13  &  454  &  0.65  & 45.6  & 1.2  & 2.9$\times 10^5$  \\ 
Oph-Bolo 21  &  16 27 33.1  &  -24 26 49  &  527  &  0.61  & 46.0  & 1.1  & 3.5$\times 10^5$  \\ 
Oph-Bolo 22  &  16 27 33.4  &  -24 25 57  &  496  &  0.58  & 43.7  & 1.0  & 3.1$\times 10^5$  \\ 
Oph-Bolo 23  &  16 27 36.7  &  -24 26 36  &  399  &  0.41  & 43.7  & 1.1  & 2.3$\times 10^5$  \\ 
Oph-Bolo 24  &  16 27 58.3  &  -24 33 10  &  291  &  0.24  & 40.7  & 1.2  & 1.6$\times 10^5$  \\ 
Oph-Bolo 25  &  16 28 00.1  &  -24 33 43  &  332  &  0.24  & 39.3  & 1.2  & 1.6$\times 10^5$  \\ 
Oph-Bolo 27  &  16 28 32.1  &  -24 17 43  &  168  &  0.90  & 112.8 & 1.8  & 0.9$\times 10^5$  \\ 
Oph-Bolo 28  &  16 28 57.7  &  -24 20 34  &  281  &  1.31  & 102.3 & 1.1  & 1.5$\times 10^5$  \\ 
Oph-Bolo 29  &  16 31 36.4  &  -24 00 42  &  284  &  0.30  & 44.9  & 1.1  & 1.0$\times 10^5$  \\ 
Oph-Bolo 31  &  16 31 40.0  &  -24 49 58  &  449  &  0.33  & 44.9  & 1.1  & 3.0$\times 10^5$  \\ 
Oph-Bolo 32  &  16 31 40.4  &  -24 49 26  &  445  &  0.32  & 46.8  & 1.0  & 3.0$\times 10^5$  \\ 
Oph-Bolo 34  &  16 31 58.0  &  -24 57 39  &  264  &  0.52  & 54.2  & 1.2  & 1.5$\times 10^5$  \\ 
Oph-Bolo 37  &  16 32 27.2  &  -24 29 15  &  3813 &  3.08  & 27.9  & 1.1  & 12.7$\times 10^5$   \\ 
Oph-Bolo 38  &  16 32 30.1  &  -23 55 18  &  245  &  0.78  & 108.8 & 1.3  & 1.0$\times 10^5$  \\ 
Oph-Bolo 39  &  16 32 33.3  &  -24 29 41  &  1032 &  1.81  & 60.7  & 1.1  & 5.2$\times 10^5$  \\ 
Oph-Bolo 40  &  16 32 42.3  &  -24 31 13  &  154  &  0.51  & 31.2  & 1.3  & 0.7$\times 10^5$  \\ 
Oph-Bolo 41  &  16 32 44.1  &  -24 33 22  &  204  &  0.50  & 49.0  & 1.2  & 0.7$\times 10^5$  \\ 
Oph-Bolo 42  &  16 32 49.2  &  -23 52 34  &  281  &  1.48  & 113.5 & 1.5  & 1.5$\times 10^5$  \\ 
Oph-Bolo 43  &  16 34 48.3  &  -24 37 25  &  212  &  1.03  & 101.7 & 1.2  & 1.3$\times 10^5$  \\ 
\enddata
\tablecomments{Bolocam identification is from Papers I-III.  The total mass is calculated from the total flux at 1.1~mm, assuming $T_D=10$~K.  Deconvolved angular FWHM sizes ($\theta_{dec}$) and axis ratios are derived from an elliptical gaussian fit, deconvolved by the $31\arcsec$ beam.  Mean densities are calculated in a fixed linear aperture of diameter $10^4$~AU for each source.  Note that the Ophiuchus identifications are different than Tables 1 and 2 of Paper II for Oph-Bolo~35 and above due to an adjustment of the source list, resulting in 43 rather than 44 sources (IDs are shifted by -1 for Oph-Bolo~35 and up).  
}
\end{deluxetable*}
\endinput


==> tab2.2.tex <==
\ProvidesFile{tab2.2.tex}

\begin{deluxetable*}{lccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Protostellar cores in Perseus, Serpens, and Ophiuchus\label{pstab}}
\tablehead{
\colhead{Bolocam ID } & \colhead{RA} & \colhead{Dec} & \colhead{Peak flux} & \colhead{Total mass} & \colhead{$\theta_{dec}$} & \colhead{Axis ratio} & \colhead{$n_{1e4}$} \\
\colhead{} & \colhead{(hr)} & \colhead{(deg)} & \colhead{(mJy/beam)} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{(arcsec)} & \colhead{} & \colhead{(cm$^{-3}$)}
}
\startdata
\hline
\multicolumn{8}{c}{Perseus}  \\
\hline
Per-Bolo 5  &  03 25 22.2  &  +30 45 09   &  727  &  2.55  & 47.3  & 1.8  & 6.5$\times10^5$  \\ 
Per-Bolo 8  &  03 25 35.9  &  +30 45 17   &  2241 &  5.86  & 36.6  & 1.2  & 20.6$\times10^5$  \\ 
Per-Bolo 10  &  03 25 38.4  &  +30 43 58  &  979  &  2.54  & 43.1  & 1.0  & 8.5$\times 10^5$  \\ 
Per-Bolo 18  &  03 26 36.9  &  +30 15 23  &  225  &  0.50  & 25.9  & 1.2  & 1.8$\times 10^5$  \\ 
Per-Bolo 21  &  03 27 37.5  &  +30 13 53  &  164  &  0.34  & 39.1  & 1.4  & 1.5$\times 10^5$  \\ 
Per-Bolo 22  &  03 27 39.3  &  +30 12 53  &  317  &  0.51  & 35.8  & 1.2  & 2.9$\times 10^5$  \\ 
Per-Bolo 23  &  03 27 41.7  &  +30 12 24  &  283  &  0.50  & 45.2  & 1.2  & 2.8$\times 10^5$  \\ 
Per-Bolo 24  &  03 27 47.9  &  +30 12 02  &  220  &  0.82  & 54.9  & 1.5  & 2.3$\times 10^5$  \\ 
Per-Bolo 25  &  03 28 32.1  &  +31 11 09  &  106  &  0.29  & 70.9  & 2.6  & 0.8$\times 10^5$  \\ 
Per-Bolo 27  &  03 28 33.3  &  +30 19 35  &  155  &  1.29  & 103.2 & 1.6  & 1.2$\times 10^5$  \\ 
Per-Bolo 28  &  03 28 34.0  &  +31 07 01  &  137  &  0.24  & 22.5  & 1.3  & 1.0$\times 10^5$  \\ 
Per-Bolo 29  &  03 28 36.2  &  +31 13 26  &  267  &  0.52  & 13.9  & 1.4  & 2.5$\times 10^5$  \\ 
Per-Bolo 30  &  03 28 39.0  &  +31 05 59  &  189  &  0.36  & 42.3  & 1.1  & 2.0$\times 10^5$  \\ 
Per-Bolo 31  &  03 28 39.9  &  +31 17 57  &  385  &  2.39  & 64.3  & 1.5  & 4.1$\times 10^5$  \\ 
Per-Bolo 35  &  03 28 48.4  &  +31 16 02  &  132  &  0.25  & 30.0  & 1.5  & 1.2$\times 10^5$  \\ 
Per-Bolo 36  &  03 28 48.7  &  +30 43 25  &  127  &  0.76  & 81.0  & 1.9  & 0.9$\times 10^5$  \\ 
Per-Bolo 37  &  03 28 52.1  &  +31 18 08  &  157  &  0.47  & 32.4  & 2.1  & 1.5$\times 10^5$  \\ 
Per-Bolo 38  &  03 28 55.3  &  +31 14 32  &  1224 &  4.15  & 42.8  & 1.3  & 10.7$\times10^5$  \\ 
Per-Bolo 39  &  03 28 55.3  &  +31 19 18  &  206  &  0.74  & 42.8  & 1.8  & 2.0$\times10^5$  \\ 
Per-Bolo 40  &  03 29 00.0  &  +31 21 38  &  685  &  1.75  & 48.2  & 1.2  & 6.7$\times10^5$  \\ 
Per-Bolo 41  &  03 29 00.6  &  +31 11 59  &  190  &  0.46  & 40.0  & 1.4  & 1.7$\times10^5$  \\ 
Per-Bolo 42  &  03 29 01.3  &  +31 20 33  &  1079 &  3.17  & 40.9  & 1.1  & 10.7$\times10^5$  \\ 
Per-Bolo 43  &  03 29 02.6  &  +31 15 57  &  2157 &  5.57  & 42.3  & 1.3  & 19.2$\times10^5$  \\ 
Per-Bolo 46  &  03 29 08.3  &  +31 15 11  &  741  &  3.27  & 64.6  & 1.1  & 7.8$\times10^5$  \\ 
Per-Bolo 47  &  03 29 08.9  &  +31 21 44  &  612  &  3.50  & 71.0  & 1.2  & 6.5$\times10^5$  \\ 
Per-Bolo 48  &  03 29 10.9  &  +31 13 26  &  5177 &  13.2  & 31.4  & 1.4  & 42.3$\times10^5$  \\ 
Per-Bolo 49  &  03 29 11.3  &  +31 18 25  &  835  &  2.47  & 44.2  & 1.1  & 7.9$\times 10^5$  \\ 
Per-Bolo 52  &  03 29 17.1  &  +31 27 39  &  269  &  0.98  & 53.8  & 2.3  & 2.2$\times 10^5$  \\ 
Per-Bolo 53  &  03 29 18.2  &  +31 25 17  &  336  &  1.71  & 67.5  & 1.5  & 3.2$\times 10^5$  \\ 
Per-Bolo 54  &  03 29 19.1  &  +31 23 27  &  330  &  1.54  & 50.2  & 1.7  & 3.2$\times 10^5$  \\ 
Per-Bolo 57  &  03 29 22.9  &  +31 33 17  &  224  &  0.64  & 34.8  & 1.3  & 2.1$\times 10^5$  \\ 
Per-Bolo 59  &  03 29 51.5  &  +31 39 13  &  249  &  0.64  & 38.5  & 1.2  & 2.1$\times 10^5$  \\ 
Per-Bolo 60  &  03 30 14.9  &  +30 23 37  &  125  &  0.46  & 45.1  & 1.7  & 1.1$\times 10^5$  \\ 
Per-Bolo 62  &  03 30 32.0  &  +30 26 19  &  199  &  0.99  & 64.1  & 1.2  & 1.9$\times 10^5$  \\ 
Per-Bolo 65  &  03 31 20.0  &  +30 45 30  &  522  &  0.95  & 29.7  & 1.2  & 4.7$\times 10^5$  \\ 
Per-Bolo 66  &  03 32 17.3  &  +30 49 44  &  1068 &  2.88  & 27.2  & 1.1  & 9.2$\times 10^5$  \\ 
Per-Bolo 68  &  03 32 28.1  &  +31 02 18  &  110  &  0.45  & 50.1  & 2.2  & 1.1$\times 10^5$  \\ 
Per-Bolo 76  &  03 33 11.4  &  +31 21 31  &  116  &  0.53  & 67.6  & 1.4  & 1.1$\times 10^5$  \\ 
Per-Bolo 78  &  03 33 13.2  &  +31 19 50  &  262  &  1.17  & 62.7  & 1.2  & 2.5$\times 10^5$  \\ 
Per-Bolo 79  &  03 33 15.0  &  +31 07 02  &  605  &  2.29  & 52.1  & 1.1  & 6.8$\times 10^5$  \\ 
Per-Bolo 80  &  03 33 17.8  &  +31 09 30  &  1083 &  3.84  & 56.7  & 1.3  & 9.5$\times 10^5$  \\ 
Per-Bolo 81  &  03 33 20.5  &  +31 07 37  &  1222 &  3.26  & 45.4  & 1.1  & 11.3$\times10^5$  \\ 
Per-Bolo 84  &  03 33 26.8  &  +31 06 50  &  186  &  0.59  & 55.5  & 1.1  & 1.8$\times10^5$  \\ 
Per-Bolo 90  &  03 41 09.0  &  +31 44 33  &  139  &  0.16  & \nodata  & 1.5  & 0.9$\times10^5$  \\ 
Per-Bolo 102  &  03 43 50.5  &  +32 03 17  &  432  &  1.76  & 60.2  & 1.2  & 4.4$\times 10^5$  \\ 
Per-Bolo 103  &  03 43 55.9  &  +32 00 46  &  994  &  3.02  & 39.0  & 1.2  & 9.0$\times 10^5$  \\ 
Per-Bolo 104  &  03 43 57.3  &  +32 03 04  &  777  &  1.78  & 38.0  & 1.2  & 7.4$\times 10^5$  \\ 
Per-Bolo 106  &  03 44 01.6  &  +32 02 02  &  426  &  0.63  & 42.4  & 1.1  & 4.2$\times 10^5$  \\ 
Per-Bolo 108  &  03 44 02.3  &  +32 04 57  &  139  &  0.40  & 51.9  & 1.4  & 1.2$\times 10^5$  \\ 
Per-Bolo 109  &  03 44 05.0  &  +32 00 28  &  127  &  0.48  & 52.7  & 1.6  & 1.1$\times 10^5$  \\ 
Per-Bolo 110  &  03 44 05.2  &  +32 02 06  &  257  &  0.54  & 45.4  & 1.1  & 3.0$\times 10^5$  \\ 
Per-Bolo 113  &  03 44 22.6  &  +31 59 23  &  122  &  0.93  & 85.1  & 1.5  & 1.2$\times 10^5$  \\ 
Per-Bolo 116  &  03 44 43.9  &  +32 01 25  &  289  &  0.63  & 21.0  & 1.3  & 2.7$\times 10^5$  \\ 
Per-Bolo 120  &  03 45 48.1  &  +32 24 15  &  83   &  0.10  & \nodata  & 1.0  & 0.5$\times10^5$  \\ 
Per-Bolo 122  &  03 47 40.8  &  +32 51 57  &  262  &  1.67  & 67.7  & 1.4  & 2.7$\times10^5$  \\ 
\hline
\multicolumn{8}{c}{Serpens}  \\
\hline
Ser-Bolo 2  &  18 28 44.0  &  +00 53 03  &  198  &  0.69  & 46.1  & 1.2  & 1.0$\times 10^5$  \\ 
Ser-Bolo 3  &  18 28 45.8  &  +00 51 32  &  227  &  0.52  & 35.3  & 1.3  & 1.1$\times 10^5$  \\ 
Ser-Bolo 7  &  18 28 53.0  &  +00 19 04  &  119  &  0.22  & 39.0  & 1.2  & 0.6$\times 10^5$  \\ 
Ser-Bolo 8  &  18 28 55.2  &  +00 29 28  &  617  &  3.55  & 59.2  & 1.2  & 3.2$\times 10^5$  \\ 
Ser-Bolo 9  &  18 28 55.9  &  +00 48 30  &  141  &  0.23  & 31.9  & 1.6  & 0.7$\times 10^5$  \\ 
Ser-Bolo 13  &  18 29 00.2  &  +00 30 20  &  239  &  0.48  & 44.7  & 1.1  & 1.2$\times 10^5$  \\ 
Ser-Bolo 14  &  18 29 07.0  &  +00 30 42  &  1016 &  2.92  & 38.3  & 1.1  & 4.8$\times 10^5$  \\ 
Ser-Bolo 15  &  18 29 09.6  &  +00 31 37  &  626  &  1.16  & 36.8  & 1.3  & 3.0$\times 10^5$  \\ 
Ser-Bolo 17  &  18 29 16.4  &  +00 18 15  &  82   &  0.54  & 81.7  & 1.2  & 0.4$\times 10^5$  \\ 
Ser-Bolo 20  &  18 29 31.9  &  +01 19 01  &  337  &  2.12  & 82.3  & 1.0  & 1.7$\times 10^5$  \\ 
Ser-Bolo 22  &  18 29 48.8  &  +01 16 51  &  1694 &  5.10  & 39.9  & 1.2  & 8.1$\times 10^5$  \\ 
Ser-Bolo 23  &  18 29 50.2  &  +01 15 25  &  3010 &  7.98  & 33.2  & 1.0  & 13.2$\times10^5$  \\ 
Ser-Bolo 24  &  18 29 53.8  &  +00 36 10  &  202  &  0.54  & 38.0  & 1.2  & 1.0$\times 10^5$  \\ 
Ser-Bolo 25  &  18 29 57.4  &  +01 13 15  &  1981 &  4.31  & 34.1  & 1.2  & 9.5$\times 10^5$  \\ 
Ser-Bolo 26  &  18 29 59.2  &  +01 14 07  &  1331 &  2.56  & 41.7  & 1.2  & 6.6$\times 10^5$  \\ 
Ser-Bolo 27  &  18 30 00.3  &  +01 10 38  &  425  &  1.60  & 45.5  & 1.5  & 2.2$\times 10^5$  \\ 
Ser-Bolo 28  &  18 30 00.7  &  +01 12 57  &  1266 &  2.56  & 41.7  & 1.2  & 6.6$\times 10^5$  \\ 
Ser-Bolo 29  &  18 30 01.0  &  +01 11 49  &  979  &  3.30  & 40.9  & 1.3  & 4.9$\times 10^5$  \\ 
Ser-Bolo 32  &  18 30 05.7  &  +00 39 32  &  105  &  0.45  & 55.8  & 1.3  & 0.5$\times 10^5$  \\ 
Ser-Bolo 33  &  18 30 06.4  &  +00 42 37  &  126  &  0.17  & 16.7  & 1.1  & 0.4$\times 10^5$  \\ 
\hline
\multicolumn{8}{c}{Ophiuchus}  \\
\hline
Oph-Bolo 4  &  16 26 09.9  &  -24 20 29  &  397  &  0.15  & 43.0  & 1.1  & 1.3$\times 10^5$  \\ 
Oph-Bolo 5  &  16 26 20.7  &  -24 22 17  &  365  &  0.50  & 58.5  & 1.1  & 1.2$\times 10^5$  \\ 
Oph-Bolo 7  &  16 26 24.7  &  -24 21 08  &  407  &  0.34  & 51.2  & 1.2  & 1.2$\times 10^5$  \\ 
Oph-Bolo 8  &  16 26 27.2  &  -24 22 27  &  1382 &  1.23  & 48.9  & 1.1  & 4.4$\times 10^5$  \\ 
Oph-Bolo 9  &  16 26 27.6  &  -24 23 37  &  2696 &  2.02  & 38.5  & 1.2  & 8.8$\times 10^5$  \\ 
Oph-Bolo 11  &  16 26 32.6  &  -24 24 45  &  1249 &  0.54  & 39.8  & 1.1  & 4.0$\times 10^5$  \\ 
Oph-Bolo 12  &  16 27 00.7  &  -24 34 17  &  540  &  1.74  & 109.8 & 1.2  & 1.9$\times 10^5$  \\ 
Oph-Bolo 14  &  16 27 07.9  &  -24 36 54  &  261  &  0.37  & 76.9  & 1.6  & 0.6$\times 10^5$  \\ 
Oph-Bolo 17  &  16 27 22.3  &  -24 27 36  &  404  &  0.32  & 52.2  & 1.2  & 1.2$\times 10^5$  \\ 
Oph-Bolo 18  &  16 27 25.2  &  -24 40 29  &  472  &  1.17  & 114.6 & 1.6  & 1.3$\times 10^5$  \\ 
Oph-Bolo 19  &  16 27 27.0  &  -24 26 57  &  615  &  0.25  & 45.5  & 1.1  & 2.3$\times 10^5$  \\ 
Oph-Bolo 20  &  16 27 29.1  &  -24 27 11  &  691  &  0.27  & 42.9  & 1.1  & 2.3$\times 10^5$  \\ 
Oph-Bolo 26  &  16 28 21.0  &  -24 36 00  &  225  &  0.51  & 114.8 & 1.2  & 0.6$\times 10^5$  \\ 
Oph-Bolo 30  &  16 31 37.2  &  -24 01 52  &  289  &  0.14  & 39.0  & 1.2  & 0.5$\times 10^5$  \\ 
Oph-Bolo 33  &  16 31 52.6  &  -24 58 01  &  204  &  0.18  & 49.3  & 1.2  & 0.5$\times 10^5$  \\ 
Oph-Bolo 35  &  16 32 00.6  &  -24 56 14  &  189  &  0.14  & 63.3  & 1.2  & 0.4$\times 10^5$  \\ 
Oph-Bolo 36  &  16 32 24.3  &  -24 28 49  &  4624 &  1.16  & 17.6  & 1.3  & 4.7$\times 10^5$  \\ 
\enddata
%\tablenotetext{1}{}
\tablecomments{Table columns are as for Table~\ref{sltab}.
Note that the Ophiuchus identifications are different than Tables 1 and 2 of Paper II for Oph-Bolo~35 and above due to an adjustment of the source list, resulting in 43 rather than 44 sources.  The peak flux, total mass, sizes, etc. for Oph-Bolo~35 and Oph-Bolo~36 are also different than in Paper~II.}
\end{deluxetable*}
\endinput


==> tab4.tex <==
\ProvidesFile{tab4.tex}

\begin{deluxetable}{lccccc}
\tablecaption{\label{vmtab} Dynamical Properties of Perseus Cores}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablehead{
\colhead{Bolocam ID} & \colhead{$T_{K}$} & \colhead{$R$} &
\colhead{$\sigma_{\mathrm{H2}}$} & \colhead{$M_{dust}$} &
\colhead{$M_{\mathrm{vir}}$}\\
\colhead{} & \colhead{(K)} & \colhead{($10^3$ AU)} &
\colhead{(km~s$^{-1}$)} & \colhead{($M_{\odot}$)} &
\colhead{($M_{\odot}$)}
}
\startdata
Per-Bolo 1 & 9.2 & 3.8 & 0.20 &     0.3 &  0.7 \\
Per-Bolo 2 & 9.2 & 2.0 & 0.23 &     0.4 &  0.4 \\
Per-Bolo 3 & 10.0 & 10.7 & 0.22 &   0.9 &   2.4 \\
Per-Bolo 4 & 10.3 & 13.1 & 0.22 &    2.8 &   2.9 \\
Per-Bolo 5 & 12.1 & 5.9 & 0.26 &     2.6 &   1.7 \\
Per-Bolo 6 & 9.1 & 13.2 & 0.21 &     3.4 &   2.5 \\
Per-Bolo 11 & 11.2 & 9.1 & 0.27 &    1.8 &   2.9 \\
Per-Bolo 13 & 9.1 & 4.8 & 0.22 &     1.4 &   1.1 \\
Per-Bolo 14 & 9.0 & 4.8 & 0.23 &     1.2 &   1.1 \\
Per-Bolo 18 & 11.7 & 3.2 & 0.24 &   0.5 &  0.8 \\
Per-Bolo 19 & 10.4 & 10.4 & 0.23 &   1.3 &   2.5 \\
Per-Bolo 20 & 10.7 & 10.1 & 0.22 &   1.5 &   2.3 \\
Per-Bolo 21 & 11.7 & 4.9 & 0.25 &   0.3 &   1.5 \\
Per-Bolo 23 & 11.4 & 5.7 & 0.25 &   0.5 &   1.6 \\
Per-Bolo 24 & 11.9 & 6.9 & 0.28 &   0.8 &   2.5 \\
Per-Bolo 25 & 10.8 & 8.9 & 0.24 &   0.3 &   2.3 \\
Per-Bolo 26 & 10.6 & 8.2 & 0.23 &    1.2 &   2.0 \\
Per-Bolo 27 & 10.7 & 12.9 & 0.23 &   1.3 &   2.9 \\
Per-Bolo 28 & 10.5 & 2.8 & 0.21 &   0.2 &  0.5 \\
Per-Bolo 30 & 10.5 & 5.3 & 0.24 &   0.4 &   1.3 \\
Per-Bolo 31 & 11.7 & 8.1 & 0.27 &    2.4 &   2.7 \\
Per-Bolo 33 & 10.5 & 5.8 & 0.24 &   0.6 &   1.5 \\
Per-Bolo 35 & 11.3 & 3.8 & 0.22 &   0.2 &  0.8 \\
Per-Bolo 37 & 13.8 & 4.1 & 0.28 &   0.5 &   1.5 \\
Per-Bolo 39 & 14.5 & 5.4 & 0.27 &   0.7 &   1.7 \\
Per-Bolo 41 & 12.5 & 5.0 & 0.29 &   0.5 &   1.9 \\
Per-Bolo 45 & 12.6 & 6.6 & 0.29 &    2.2 &   2.4 \\
Per-Bolo 49 & 14.3 & 5.5 & 0.31 &    2.5 &   2.3 \\
Per-Bolo 52 & 11.8 & 6.7 & 0.23 &   1.0 &   1.6 \\
Per-Bolo 53 & 13.4 & 8.5 & 0.23 &    1.7 &   2.0 \\
Per-Bolo 54 & 13.3 & 6.3 & 0.25 &    1.5 &   1.7 \\
Per-Bolo 56 & 9.8 & 10.5 & 0.22 &    1.5 &   2.3 \\
Per-Bolo 57 & 10.4 & 4.4 & 0.22 &   0.6 &  0.9 \\
Per-Bolo 58 & 10.3 & 3.2 & 0.22 &   0.7 &  0.7 \\
Per-Bolo 59 & 10.5 & 4.8 & 0.22 &   0.6 &   1.1 \\
Per-Bolo 60 & 11.0 & 5.7 & 0.23 &   0.5 &   1.3 \\
Per-Bolo 61 & 10.5 & 8.6 & 0.20 &   0.8 &   1.6 \\
Per-Bolo 62 & 10.0 & 8.0 & 0.23 &   1.0 &   1.9 \\
Per-Bolo 63 & 10.5 & 9.9 & 0.23 &    1.5 &   2.4 \\
Per-Bolo 64 & 9.8 & 4.6 & 0.20 &    0.5 &  0.8 \\
Per-Bolo 65 & 11.4 & 3.7 & 0.26 &   1.0 &   1.2 \\
Per-Bolo 67 & 10.5 & 8.0 & 0.24 &    1.9 &   2.0 \\
Per-Bolo 68 & 9.6 & 6.3 & 0.20 &    0.5 &   1.2 \\
Per-Bolo 70 & 10.2 & 12.2 & 0.22 &   4.6 &   2.7 \\
Per-Bolo 71 & 11.2 & 10.4 & 0.29 &   2.3 &   4.1 \\
Per-Bolo 72 & 10.1 & 7.7 & 0.22 &    2.2 &   1.7 \\
Per-Bolo 74 & 10.0 & 5.6 & 0.23 &   0.9 &   1.3 \\
Per-Bolo 75 & 9.9 & 5.6 & 0.26 &    0.9 &   1.7 \\
Per-Bolo 78 & 9.4 & 7.9 & 0.21 &     1.2 &   1.6 \\
Per-Bolo 82 & 9.7 & 6.0 & 0.21 &    0.9 &   1.2 \\
Per-Bolo 89 & 12.4 & 11.9 & 0.23 &   1.7 &   2.7 \\
Per-Bolo 92 & 9.5 & 6.3 & 0.19 &    0.6 &   1.1 \\
Per-Bolo 94 & 9.6 & 6.6 & 0.20 &    0.8 &   1.2 \\
Per-Bolo 100 & 12.3 & 6.7 & 0.24 &   1.4 &   1.7 \\
Per-Bolo 101 & 14.8 & 5.6 & 0.25 &  0.4 &   1.6 \\
Per-Bolo 102 & 11.7 & 7.5 & 0.27 &   1.8 &   2.5 \\
Per-Bolo 103 & 12.9 & 4.9 & 0.30 &   3.0 &   2.0 \\
Per-Bolo 105 & 12.9 & 5.8 & 0.27 &  1.0 &   1.9 \\
Per-Bolo 107 & 11.1 & 5.8 & 0.26 &  1.0 &   1.7 \\
Per-Bolo 109 & 10.7 & 6.6 & 0.28 &  0.5 &   2.4 \\
Per-Bolo 110 & 10.9 & 5.7 & 0.24 &  0.5 &   1.5 \\
Per-Bolo 111 & 10.6 & 9.7 & 0.23 &   1.8 &   2.3 \\
Per-Bolo 112 & 12.9 & 6.7 & 0.25 &  0.7 &   2.0 \\
Per-Bolo 113 & 10.5 & 10.7 & 0.24&  0.9 &   2.7 \\
Per-Bolo 115 & 10.8 & 6.6 & 0.25 &   1.1 &   1.9 \\
Per-Bolo 117 & 10.8 & 5.4 & 0.22 &  0.8 &   1.2 \\
Per-Bolo 118 & 10.9 & 6.6 & 0.23 &  0.7 &   1.6 \\
Per-Bolo 119 & 10.7 & 12.7 & 0.21&   2.8 &   2.5 \\
Per-Bolo 121 & 10.0 & 10.4 & 0.20&   1.6 &   2.0 \\
Per-Bolo 122 & 11.7 & 8.5 & 0.25 &   1.7 &    2.4 
\enddata
\tablecomments{Kinetic temperatures ($T_K$) and linewidths ($\sigma_{\mathrm{H2}}$) are derived from the NH$_3$ observations of Perseus cores completed by \citet{ros07}.  The virial mass $M_{\mathrm{vir}}$ is calculated according to Eq.~\ref{vireq}, with the effective radius $R$ estimated as the deconvolved HWHM of the 1.1~mm identified core ($\theta_{dec}/2$).  $M_{\mathrm{dust}}$ is the mass calculated from the total 1.1~mm flux (Tables~\ref{sltab} and \ref{pstab}).}
\end{deluxetable}

\endinput

